Deep Learning for Chest X-ray Analysis: A Survey

Recent advances in deep learning have led to a promising performance in many medical image analysis tasks. As the most commonly performed radiological exam, chest radiographs are a particularly important modality for which a variety of applications have been researched. The release of multiple, large, publicly available chest X-ray datasets in recent years has encouraged research interest and boosted the number of publications. In this paper, we review all studies using deep learning on chest radiographs, categorizing works by task: image-level prediction (classification and regression), segmentation, localization, image generation and domain adaptation. Commercially available applications are detailed, and a comprehensive discussion of the current state of the art and potential future directions are provided.

==> tables/commercial_table_old.tex <==
\afterpage{\onecolumn
\scriptsize

\begin{longtable}{p{2.3cm}p{3.4cm}p{4.9cm}p{2.9cm}p{2.6cm}}
\caption{Commercial Products for CXR analysis. (Section \ref{sec:commercial}) \\ \textbf{Labels}: T=Triage/Abnormal, PM=Pneumonia, CV=COVID, TB=Tuberculosis, LO=Lesion or Opacity, CM=Cardiomegaly, ND=Nodule, PE=Effusion, PT=Pneumothorax, TU=Catheter or Tube, LC=Lung Cancer, BS=Bone Suppression, E=Edema, Z=Other\\ \textbf{Output}: LOC=Localization, PRI=Prioritization, REP=Report, SCOR=Scoring}\label{tab:commercial}\\
\toprule
       Company & Product & Literature (4 most recent) & Labels (Total number) & Output\\
\midrule
\endhead
\midrule
\multicolumn{5}{r} {{Continued on next page}} \\

\midrule
\endfoot

\bottomrule
\endlastfoot
Siemens Healthineers & AI-Rad Companion Chest X-Ray & ~\cite{Fisc20} & LO PE PT Z (5) &  LOC, SCOR, REP \\
Samsung Healthcare &	Auto Lung Nodule Detection & 	~\cite{Sim19} & ND (1) & LOC\\
Thirona	& CAD4COVID-XRay	& ~\cite{Murp20} &  CV (1) & LOC, SCOR\\
Thirona & 	CAD4TB &	~\cite{Murp20a, Habi20, Qin19,  Sant20} & TB (1) & LOC, SCOR\\
Oxipit &	ChestEye CAD & & T (1)  & REP (healthy) \\	
Arterys & 	Chest $|$ MSK AI	& & LO, ND, PE, PT (4) & LOC, SCOR, PRI\\
Quibim	& Chest X-Ray Classifier	&~\cite{Lian20} &  PM  CM  ND  PE  PT  E  Z (16) & LOC, SCOR, REP\\ 
GE	& Critical Care Suite  & & PT (1) & LOC, SCOR\\	
InferVision	& InferRead DR Chest & &  TB  PE  PT  LC  Z (9)  & LOC, SCOR\\	
JLK	& JLD-O2K  & &  LC  Z (16) & LOC, SCOR\\	
Lunit &	Lunit INSIGHT CXR	&~\cite{Hwan19, Hwan19a, Hwan19b, Qin19}&  TB  CM  ND  PE  PT  Z (11) & LOC, SCOR, PRI, REP\\
qure.ai	& qXR	& ~\cite{Sing18, Nash20, Engl20, Qin19} &  T  CV  TB  Z (30) & LOC, SCOR, PRI, REP\\
Digitec	& TIRESYA & &  BS (1) & Bone Suppressed Image\\	
VUNO &	VUNO Med-Chest X-Ray& 	~\cite{Kim17} &  LO  ND  PE  PT  Z (5) & LOC, SCOR\\
Riverain Technologies	& ClearRead Xray - Bone Suppress &	~\cite{Homa20, Dell17, Scha16, Scha14}& BS(1) & Bone Suppressed Image\\
Riverain Technologies	& ClearRead Xray - Compare	& & LC(1) & Subtraction Image\\
Riverain Technologies	& ClearRead Xray - Confirm	& & TU(1) & LOC\\
Riverain Technologies	& ClearRead Xray - Detect	& ~\cite{Dell17, Scha14a, Szuc13}& ND LC (2) & LOC\\
behold.ai	& Red Dot	& & T PT (2) & LOC\\
Zebra Medical Vision &	Triage Pleural Effusion	& & PE & LOC, PRI\\
Zebra Medical Vision &	Triage Pneumothorax	& & PT & LOC, PRI\\
\end{longtable}


\twocolumn}


%\begin{longtable}{p{3.6cm}p{3.6cm}p{4.5cm}p{1.5cm}p{1.5cm}}
%\caption{Commercial}\label{tab:commercial}\\
%\toprule
%       Company & Product (website) & Literature & Labels (Total Labels) & Output\\
%\midrule
%\endhead
%\midrule
%\multicolumn{5}{r}{{Continued on next page}} \\
%\midrule
%\endfoot

%\bottomrule
%\endlastfoot

% Siemens Healthineers & AI-Rad Companion Chest X-Ray~\citep{siem21} & ~\cite{Fisc20} & LO PE PT Z (5) &  Localization \\
%\end{longtable}


